I See, Therefore I Do: Estimating Causal Effects for Image Treatments

Causal effect estimation under observational studies is challenging due to the lack of ground truth data and treatment assignment bias. Though various methods exist in literature for addressing this problem, most of them ignore multi-dimensional treatment information by considering it as scalar, either continuous or discrete. Recently, certain works have demonstrated the utility of this rich yet complex treatment information into the estimation process, resulting in better causal effect estimation. However, these works have been demonstrated on either graphs or textual treatments. There is a notable gap in existing literature in addressing higher dimensional data such as images that has a wide variety of applications. In this work, we propose a model named NICE (Network for Image treatments Causal effect Estimation), for estimating individual causal effects when treatments are images. NICE demonstrates an effective way to use the rich multidimensional information present in image treatments that helps in obtaining improved causal effect estimates. To evaluate the performance of NICE, we propose a novel semi-synthetic data simulation framework that generates potential outcomes when images serve as treatments. Empirical results on these datasets, under various setups including the zero-shot case, demonstrate that NICE significantly outperforms existing models that incorporate treatment information for causal effect estimation.

==> algorithm.tex <==
\section{algorithm}
% Algorithm code
\begin{algorithm}
\caption{CIME Training}
\begin{algorithmic}
\STATE \textbf{Input:} Observational data: \( \mathcal{D} = \{ (x_i, t_i, y_{t_i}^i) \}_{i=1}^N \sim \mathcal{D}_{\text{train}} \), and hyperparameters \( \alpha \geq 0 \) and \( \beta \geq 0 \).
\STATE \textbf{Output:} An outcome prediction model consisting of Treatment Head Networks: \(f \rightarrow \pi_k = (\phi(x), \psi(t_{\text{obs}})) \)
\STATE Initialize parameters: \( \phi, \psi, \pi \)
\WHILE{{\textit{not converged}}}
    \STATE Sample a mini-batch \( B = \{ (x_{i_o}, t_{i_o}, y_{t_{i_o}}^{i_o}) \}_{o=1}^B \subset \mathcal{D}_{\text{train}} \)
    \STATE Mini-batch approximation of Regression Loss \(\mathcal{L}_1\):
    \STATE Compute:
    \[
    \mathcal{L}_1 = \frac{1}{|B|} \sum_{o=1}^{|B|} (\hat{y}_{t_{i_o}}^{i_o} - y_{t_{i_o}}^{i_o})^2
    \]
    \STATE Mini-batch approximation of the Treatment Regularization Loss \(\mathcal{L}_2\):
    \[
    \mathcal{L}_2 = \Pi(\phi(x), \psi(t_{\text{obs}}))
    \]
    \STATE \textbf{Update Functions}:
    \[
    \phi, \psi, \pi_k \leftarrow \phi - \lambda \nabla_{\phi} (\alpha \cdot \mathcal{L}_1 + \beta \cdot \mathcal{L}_2), \psi - \lambda \nabla_{\psi} (\alpha \cdot \mathcal{L}_1 + \beta \cdot \mathcal{L}_2), \pi_k - \lambda \nabla_{\pi_k} (\alpha \cdot \mathcal{L}_1 + \beta \cdot \mathcal{L}_2)
    \]
    \STATE \textbf{Minimize}:
    \[
    \alpha \cdot \mathcal{L}_1 + \beta \cdot \mathcal{L}_2
    \]
    using SGD
\ENDWHILE
\end{algorithmic}
\end{algorithm}


==> tables.tex <==
%% Hyperparam table
\begin{table}[h!]
\centering
\begin{tabular}{c|c}
\hline
\textbf{Hyperparameter} & \textbf{Search Range} \\
\hline
Number of layers ($\phi$) & \{4, 6, 8\} \\
\hline
Number of nodes ($\phi$) & \{200, 400, 600\} \\
\hline
Number of layers ($\psi$) & \{4, 6, 8\} \\
\hline
Number of nodes ($\psi$) & \{200, 400, 600\} \\
\hline
Number of layers ($\pi$) & \{4, 6, 8\} \\
\hline
Number of nodes ($\pi$) & \{200, 400, 600\} \\
\hline
Batch Size & \{512\} \\
\hline
Alpha $\alpha$ & \{0.5, 1.0\} \\
\hline
Beta $\beta$ & \{0.5\} \\
\hline
Batch Size & \{512\} \\
\hline
Learning Rate & \{0.1, 0.01\} \\
\hline
Learning rate Decay & \{1e$^{-1}$\} \\
\hline
Learning Scheduler Step & \{10, 15\} \\
\hline
Weight Decay & \{1e$^{-4}$\} \\
\hline
Dropout & \{0.1\} \\
\hline
Activation & \{TanH, ELU\} \\
\hline
\end{tabular}
\caption{Hyperparameter search range for \textbf{NICE} (our proposed method) and baselines on semi-synthetic datasets.}
\label{tab:hyperparameter_search}
\end{table}


%%% PEHE table
\begin{table*}[ht]
\centering
\caption{Performance comparison of different methods on semi-synthetic datasets using images as treatments, with variations in the number of treatments. The comparison is based on the Rooted \textbf{P}recision in the \textbf{E}stimation of \textbf{H}eterogeneous \textbf{E}ffects (PEHE) metric. Bold results indicate the best performance for each treatment.}

\label{tab:pehe_comparison}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Treatment = 4} & \textbf{Treatment = 8} & \textbf{Treatment = 16} \\
\hline
Naive & 139.33 $\pm$ 22.84 & 148.42  $\pm$ 29.7 & 155.04 $\pm$ 17.16 \\
TarNet & 128.25 $\pm$ 24.07 & 137.67 $\pm$ 26.75 & 152.77 $\pm$ 15.69 \\
GraphITE & 128.26 $\pm$ 24.52 & 135.33 $\pm$ 22.13 & 141.06 $\pm$ 12.76 \\
SIN & 127.74 $\pm$ 24.71 & 134.68 $\pm$ 22.06 & 139.92 $\pm$ 12.9 \\
CaML & 127.74 $\pm$ 24.71 & 138.0 $\pm$ 20.63 & 139.72 $\pm$ 13.05 \\
\rowcolor{gray!20}
\textbf{NICE - ResNet} & \textbf{91.95 $\pm$ 12.06} & \textbf{105.22 $\pm$ 14.92} & 114.38 $\pm$ 10.16 \\
\hline
\rowcolor{gray!20}
\textbf{NICE - VGG} & 98.95 $\pm$  13.16 & 107.57 $\pm$ 17.61 & \textbf{113.94 $\pm$ 9.97} \\
\hline
\end{tabular}
\end{table*}

%%% PEHE table zero shot 
\begin{table*}[ht]
\centering
\caption{Performance comparison of NICE in a zero-shot setting against baselines, with variations in treatment to assess causal estimation on unseen treatments. The comparison is evaluated using the Rooted PEHE ($\sqrt{\epsilon \text{PEHE}}$) metric. Bolded values indicate the best performance for each treatment.}

\label{tab:pehe_comparison_zero_shot}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Treatment = 4} & \textbf{Treatment = 8} & \textbf{Treatment = 16} \\
\hline
TarNet & ip $\pm$ ip & ip $\pm$ ip & ip $\pm$ ip\\
GraphITE & 128.35 $\pm$ 25.24 & 136.68 $\pm$ 19.29 & 145.13 $\pm$ 23.59 \\
SIN        ip  & ip $\pm$ ip & ip $\pm$ ip & ip $\pm$ ip \\
CaML & 120.68 $\pm$ 24.55 & 133.38 $\pm$  17.84 & 135.89 $\pm$ 13.97 \\
\rowcolor{gray!20}
\textbf{NICE - ResNet} & \textbf{92.74 $\pm$ 15.64} & \textbf{103.82 $\pm$10.79} &117.78$\pm$16.82 \\
\hline
\rowcolor{gray!20}
\textbf{NICE - VGG} & 98.61 $\pm$ 17.22& 106.79 $\pm$13.09 & \textbf{117.37 $\pm$17.77} \\
\hline
\end{tabular}
\end{table*}


%%% PEHE table kappa 50
\begin{table*}[ht]

\caption{Performance comparison of NICE against baselines under varying treatment assignment bias $\kappa= 50$, introducing skewness in treatment assignment to better reflect real-world scenarios. The comparison is evaluated using the Rooted PEHE ($\sqrt{\epsilon \text{PEHE}}$) metric. Bolded values indicate the best performance for each treatment.}

\label{tab:pehe_comparison_kappa_50}
\begin{tabular}{lccc}
\centering
\hline
\textbf{Method} & \textbf{Treatment = 4} & \textbf{Treatment = 8} & \textbf{Treatment = 16} \\
\hline
Naive & 139.33 $\pm$ 22.84 & 148.42  $\pm$ 29.7 & 155.04 $\pm$ 17.16 \\
TarNet & 128.25 $\pm$ 24.07 & 137.67 $\pm$ 26.75 & 152.77 $\pm$ 15.69 \\
GraphITE & 128.26 $\pm$ 24.52 & 135.33 $\pm$ 22.13 & 141.06 $\pm$ 12.76 \\
SIN & 127.74 $\pm$ 24.71 & 134.68 $\pm$ 22.06 & 139.92 $\pm$ 12.9 \\
CaML & 127.74 $\pm$ 24.71 & 138.0 $\pm$ 20.63 & 139.72 $\pm$ 13.05 \\
\rowcolor{gray!20}
\textbf{NICE - ResNet} & \textbf{91.95 $\pm$ 12.06} & \textbf{105.22 $\pm$ 14.92} & 114.38 $\pm$ 10.16 \\
\hline
\rowcolor{gray!20}
\textbf{NICE - VGG} & 98.95 $\pm$  13.16 & 107.57 $\pm$ 17.61 & \textbf{113.94 $\pm$ 9.97} \\
\hline
\end{tabular}
\end{table*}

%%% PEHE table kappa 100
\begin{table*}[ht]
\centering
\caption{Performance comparison of NICE against baselines under varying treatment assignment bias $\kappa= 100$, introducing skewness in treatment assignment to better reflect real-world scenarios. The comparison is evaluated using the Rooted PEHE ($\sqrt{\epsilon \text{PEHE}}$) metric. Bolded values indicate the best performance for each treatment.}

\label{tab:pehe_comparison_kappa_100}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Treatment = 4} & \textbf{Treatment = 8} & \textbf{Treatment = 16} \\
\hline
Naive & 131.59 $\pm$ 22.63 & 146.45 $\pm$ 26.45 & 155.67 $\pm$ 18.83 \\
TarNet & 131.9 $\pm$ 25.79 & 139.65 $\pm$ 22.69 & 148.98 $\pm$ 18.57\\
GraphITE & 129.28 $\pm$ 24.33 & 142.99 $\pm$ 21.05 & 148.79 $\pm$ 13.15 \\
SIN          & ip $\pm$ ip & ip $\pm$ ip & ip $\pm$ ip \\
CaML & 127.74 $\pm$ 24.71 & 134.24 $\pm$ 21.83 & 135.39  $\pm$ 8.45 \\
\rowcolor{gray!20}
\textbf{NICE - ResNet} & 103.49 $\pm$ 41.21 & \textbf{107.49 $\pm$18.35} &\textbf{129.59 $\pm$23.84} \\
\hline
\rowcolor{gray!20}
\textbf{NICE - VGG} & \textbf{96.08 $\pm$ 13.16}& 108.6 $\pm$ 18.2 & 131.93$\pm$19.58 \\
\hline
\end{tabular}
\end{table*}
